Mapping tori of $A_{\infty}$-autoequivalences and Legendrian lifts of exact Lagrangians in circular contactizations

We study mapping tori of quasi-autoequivalences $\tau : \mathcal{A} \to \mathcal{A}$ which induce a free action of $\mathbf{Z}$ on objects. More precisely, we compute the mapping torus of $\tau$ when it is strict and acts bijectively on hom-sets, or when the $A_{\infty}$-category $\mathcal{A}$ is directed and there is a bimodule map $\mathcal{A} (-, -) \to \mathcal{A} (-, \tau (-))$ satisfying some hypotheses. Then we apply these results in order to link together the Fukaya $A_{\infty}$-category of a family of exact Lagrangians, and the Chekanov-Eliashberg DG-category of Legendrian lifts in the circular contactization.

==> Ekholm_Lekili/ekholm_lekili.tex <==
% !TeX spellcheck = en_US
\chapter{Ekholm-Lekili revisited}\label{section EL}

In this appendix, we revisit some of the results of \cite{EL21} using localization of $A_{\infty}$-categories. 

\section{Setting}

Let $X$ be a Weinstein manifold. 
%We will assume that the induced contact form $\alpha$ on $Y = \partial_{\infty} X$ is hypertight. 
Now let $L$ be a connected cylindrical exact Lagrangian submanifold of $X$. We denote by $\Lambda = \partial_{\infty} L \subset Y$ the corresponding Legendrian submanifold. We will assume that $\Lambda$ is connected and chord generic with respect to $\alpha$. Finally, we denote by $\varepsilon_L : CE_{-*} \left( \Lambda \right) \to \mathbf{F}$ the augmentation induced by $L$. 

We fix two positive Morse functions $F_1 : L \to \mathbf{R}$ and $f_1 : \Lambda \to \mathbf{R}$ with a unique minimum and a unique maximum, and such that in the ends 
\[F_1 \left( t,q \right) = a_1 \left( t + f_1 \left( q \right) \right) + b_1 \text{ for } 0 < a_1 \ll 1 \text{ and } b_1 > 0. \]
We denote by $\mcU$ a small open neighborhood of $\left( F_1, f_1 \right)$ in $C^{\infty} \left( L \right) \times C^{\infty} \left( \Lambda \right)$ with the following property: for every pair $\left( F, f \right)$ in $\mcU$, the functions $F$, $f$ are positive, Morse, and their critical points and gradient trajectories are in bijection with those of $F_1$, $f_1$ respectively. 
Then we choose a family $\left( F_n, f_n \right)_{n \geq 2}$ of pairs in $\mcU$ such that in the ends,
\[F_n \left( t,q \right) = a_n \left( t + f_n \left( q \right) \right) + b_n \text{ for } 0 < a_n \ll 1 \text{ and } b_n > 0. \]
We also choose a decreasing sequence $\left( \delta_k \right)_{k \geq 1}$ of small enough positive numbers so that the family
\[\left( H_n = \sum_{k=1}^{n} \delta_k F_k, h_n = \sum_{k=1}^{n} \delta_k f_k \right)_{n \in \mathbf{N}} \]
has the following property: for every $i<j$, the pair $\left( H_j - H_i, h_j - h_i \right)$ lies in the cone over $\mcU$ (this can be easily achieved by induction on $n$).
Finally, we let $L_n \subset X$ be the Lagrangian corresponding to the graph of $d H_n$ in a Weinstein neighborhood of $L = L_0$, and we let $\Lambda_n \subset Y$ be the Legendrian corresponding to the one-jet of $h_n$ in a Weinstein neighborhood of $\Lambda = \Lambda_0$. Observe that we \emph{do not} require the copies to be parallel in the sense of the third item of Lemma 31 (or Theorem 76) in \cite{EL21}.

\section{Some $A_{\infty}$-categories}

%\begin{rmk}
%	
%	Let $\eta$ be the length of the smallest Reeb chord of $\Lambda$. The set $\mcR \left( \Lambda_i, \Lambda_j \right)$ of Reeb chords starting on $\Lambda_i$ and ending on $\Lambda_j$ splits as 
%	\[\mcR \left( \Lambda_i, \Lambda_j \right) = \mcR_{long} \left( \Lambda_i, \Lambda_j \right) \sqcup \mcR_{short} \left( \Lambda_i, \Lambda_j \right), \]
%	where $\mcR_{long} \left( \Lambda_i, \Lambda_j \right)$ is the set of chords with length greater than $\eta / 2$ (and $\mcR_{short} \left( \Lambda_i, \Lambda_j \right)$ is the complementary set). In the following, we choose the numbers $\delta_k$ small enough so that the maximum of $h_n$ is very small compare to $\eta$.
%	
%\end{rmk}

%\begin{defin}\label{definition positive augmentation category}
%	
%	Let $\mcA_+$ be the $A_{\infty}$-category such that
%	\begin{enumerate}
%		
%		\item the set of objects of $\mcA_+$ is $\{ \Lambda_n \mid n \in \mathbf{N} \}$,
%		
%		\item the space of morphisms from $\Lambda_i$ to $\Lambda_j$ is either $\langle \mcR \left( \Lambda_i, \Lambda_j \right) \rangle$ if $i \ne j$, or $\mathbf{F} \oplus \mcR \left( \Lambda_i \right)$ if $i=j$, and
%		
%		\item the operations count punctured pseudo-holomorphic discs in $\mathbf{R} \times Y$ with boundary on $\bigcup\limits_{n \in \mathbf{N}} \mathbf{R} \times \Lambda_n$, asymptotic to Reeb chords at punctures, and anchored in $\left( X,L \right)$. \textcolor{red}{Détailler. Dynamically convex?}
%		
%	\end{enumerate}
%	Besides, let $W_+$ be the set made of the morphisms $c_n \in \mcA_+ \left( \Lambda_n, \Lambda_{n+1} \right)$ corresponding to the minimum of $\left( h_{n+1} - h_n \right)$ for $n \in \mathbf{N}$.
%	We define
%	\[LA_+^* \left( \Lambda \right) := \mathrm{End}_{\mcA_+ \left[ W_+^{-1} \right]} \left( \Lambda \right) . \]
%	
%\end{defin}
%
%We also define a directed version, following \cite{Cha19} section 3.3. 
%
%\begin{defin}
%	
%	Let $\mcA_{++}$ be the $A_{\infty}$-category such that
%	\begin{enumerate}
%		
%		\item the set of objects of $\mcA_{++}$ is $\{ \Lambda_n \mid n \in \mathbf{N} \}$,
%		
%		\item the space of morphisms from $\Lambda_i$ to $\Lambda_j$ is either $\langle \mcR \left( \Lambda_i, \Lambda_j \right) \rangle$ if $i < j$, or $\mathbf{F}$ if $i=j$, or $0$ if $i>j$, and
%		
%		\item the operations count punctured pseudo-holomorphic discs in $\mathbf{R} \times Y$ with boundary on $\bigcup\limits_{n \in \mathbf{N}} \mathbf{R} \times \Lambda_n$, asymptotic to Reeb chords at punctures, and anchored in $\left( X,L \right)$. \textcolor{red}{Détailler}
%		
%	\end{enumerate}
%	Besides, let $W_+^{dir}$ be the set made of the morphisms $c_n \in \mcA_+ \left( \Lambda_n, \Lambda_{n+1} \right)$ corresponding to the minimum of $\left( h_{n+1} - h_n \right)$ for $n \in \mathbf{N}$.
%	
%\end{defin}
%
%\begin{rmk}
%	
%	In \cite{Cha19} section 3.3, the author defined an $A_{\infty}$-category $\mcA ug_+ \left( \Lambda \right)$. We have 
%	\[\mcA_{++} \left[ \left( W_+^{dir} \right)^{-1} \right] \simeq \mathrm{End}_{\mcA ug_+ \left( \Lambda \right)} \left( \varepsilon_L \right), \]
%	where $\varepsilon_L : CE_* \left( \Lambda \right) \to \mathbf{F}$ is the augmentation induced by $L$. 
%	
%\end{rmk}

%\begin{lemma}\label{lemma directed and non-directed positive augmentation categories}
%	
%	The natural strict $A_{\infty}$-functor $\mcA_{++} \to \mcA_+$ induces a quasi-equivalence 
%	\[\mcA_{++} \left[ \left( W_+^{dir} \right)^{-1} \right] \simeq \mcA_+ \left[ \left( W_+ \right)^{-1} \right] . \]
%	
%\end{lemma}
%
%\begin{proof}
%	
%	\textcolor{red}{Ecrire la preuve.}
%	
%\end{proof}

%\begin{lemma}\label{lemma multiplication by the minimum}
%	
%	For every integer $n$, the continuation element $c_n \in \mcR \left( \Lambda_n, \Lambda_{n+1} \right) \cap W_+$ satisfies the following. For every $m \in \mathbf{N}$, the chain maps $\mu^2 \left( c, - \right) : \mcA_{long} \left( \Lambda_{n+1}, \Lambda_m \right) \to \mcA_{long} \left( \Lambda_n, \Lambda_m \right)$ and $\mu^2 \left( -, c \right) : \mcA_{long} \left( \Lambda_m, \Lambda_n \right) \to \mcA_{long} \left( \Lambda_m, \Lambda_{n+1} \right)$ are quasi-isomorphisms (where $\mcA_{long} \left( \Lambda_i, \Lambda_j \right)$ denotes the subcomplex of $\mcA_+ \left( \Lambda_i, \Lambda_j \right)$ generated bu $\mcR_{long} \left( \Lambda_i, \Lambda_j \right)$). 
%	
%\end{lemma}
%
%\begin{proof}
%	
%	\textcolor{red}{Ecrire la preuve.}
%	
%\end{proof}

%\begin{defin}
%	
%	Let $\mcA_0$ be the $A_{\infty}$-category such that
%	\begin{enumerate}
%		
%		\item the set of objects of $\mcA_0$ is $\{ \Lambda_n \mid n \in \mathbf{N} \}$,
%		
%		\item the space of morphisms from $\Lambda_i$ to $\Lambda_j$ is either $\langle \mcR_{short} \left( \Lambda_i, \Lambda_j \right) \rangle$ if $i<j$, or $\mathbf{k}$ if $i=j$, or $0$ if $i>j$, and
%		
%		\item the operations count punctured pseudo-holomorphic discs in $\mathbf{R} \times Y$ with boundary on $\bigcup\limits_{n \in \mathbf{N}} \mathbf{R} \times \Lambda_n$, asymptotic to Reeb chords at punctures, and anchored in $\left( X,L \right)$. \textcolor{red}{Détailler}
%		
%	\end{enumerate}
%	Besides, let $W_0$ be the set made of the morphisms $c_n \in \mcA_0 \left( \Lambda_n, \Lambda_{n+1} \right)$ corresponding to the minimum of $\left( h_{n+1} - h_n \right)$ for $n \in \mathbf{N}$.
%	We define
%	\[LA_0^* \left( \Lambda \right) := \mathrm{End}_{\mcA_0 \left[ W_0^{-1} \right]} \left( \Lambda \right) . \]
%	
%\end{defin}

%Observe that the projection $\pi : \mcA_+ \to \mcA_0$ defines a strict $A_{\infty}$-functor which sends $W_+$ to $W_0$. Thus, it induces an $A_{\infty}$-map $\widetilde{\pi} : LA_+^* \left( \Lambda \right) \to LA_0^* \left( \Lambda \right)$. 
%Besides, let $\overline{LA^*} \left( \Lambda \right)$ be the Legendrian non-unital $A_{\infty}$-algebra associated to $\left( \Lambda, \varepsilon_L \right)$. It is the endomorphism algebra of $\varepsilon_L$ in the $A_{\infty}$-category $\mcA ug_- \left( \Lambda \right)$ defined in \cite{BC14}. The inclusion $\overline{LA^*} \left( \Lambda \right) \to \mcA_+ \left( \Lambda, \Lambda \right)$ induces a strict $A_{\infty}$-map $\iota : \overline{LA^*} \left( \Lambda \right) \to \ker \left( \widetilde{\pi} \right) \subset LA_+^* \left( \Lambda \right)$.
%
%\begin{prop}\label{prop Lagrangian algebra as a cone}
%	
%	The $A_{\infty}$-map $\iota : \overline{LA^*} \left( \Lambda \right) \to \ker \left( \widetilde{\pi} \right)$ induces a quasi-isomorphism 
%	\[\overline{LA^*} \left( \Lambda \right) \simeq \mathrm{Cone} \left( LA_+^* \left( \Lambda \right) \xrightarrow{\widetilde{\pi}} LA_0^* \left( \Lambda \right) \right) . \]
%	
%\end{prop}
%
%\begin{proof}
%	
%	\textcolor{red}{Revoir.}
%	
%	Observe that the inclusion $\ker \left( \widetilde{\pi} \right) \to \mathrm{Cone} (\widetilde{\pi})$ is an $A_{\infty}$-map, and it is a quasi-isomorphism because $\widetilde{\pi}$ is surjective. Thus, it suffices to show that $\ker \left( \widetilde{\pi} \right) / \mathrm{im} (\iota)$ is acyclic. We have 
%	\begin{align*}
%	\ker \left( \widetilde{\pi} \right) / \mathrm{im} (\iota) & = \ker \left( \widetilde{\pi}_{| \bigoplus\limits_{\substack{p \geq 1 \\ c_1, \dots, c_p \in W_+}} \mcA_+ \left( \Lambda_0, \mathrm{Cone} (c_1) \right) \otimes \dots \otimes \mcA_+ \left( \mathrm{Cone} (c_p), \Lambda_0 \right)} \right) \\
%	& = \bigoplus\limits_{\substack{p \geq 1 \\ c_1, \dots, c_p \in W_+}} \bigoplus_{i=0}^{p+1} \mcA_+ \left( \Lambda_0, \mathrm{Cone} (c_1) \right) \otimes \dots \otimes \ker \left( \widetilde{\pi}_{|\mcA_+ \left( \mathrm{Cone} (c_{i-1}), \mathrm{Cone} (c_i) \right)} \right) \\ 
%	& \mkern 300mu \otimes \dots \otimes \mcA_+ \left( \mathrm{Cone} (c_p), \Lambda_0 \right)
%	\end{align*}
%	%	(the second equality holds because $\widetilde{\pi}$ preserves the filtration by $p$)
%	with the convention that 
%	\[\mathrm{Cone} (c_0) = \mathrm{Cone} (c_{p+1}) = \Lambda_0. \]
%	We will show that $\ker \left( \widetilde{\pi}_{|\mcA_+ \left( \Lambda_0, \mathrm{Cone} (c) \right)} \right)$, $\ker \left( \widetilde{\pi}_{|\mcA_+ \left( \mathrm{Cone} (c), \Lambda_0 \right)} \right)$ and $\ker \left( \widetilde{\pi}_{|\mcA_+ \left( \mathrm{Cone} (c), \mathrm{Cone} (c') \right)} \right)$ are acyclic for every $c, c' \in W_+$. This will imply that $\ker \left( \widetilde{\pi} \right) / \mathrm{im} (\iota)$ is acyclic, which gives the desired result.
%	
%	Let $c \in \mcR \left( \Lambda_i, \Lambda_{i+1} \right) \cap W_+$. Then 
%	\begin{align*}
%	\ker \left( \widetilde{\pi}_{|\mcA_+ \left( \Lambda_0, \mathrm{Cone} (c) \right)} \right) & = \mcA_{long} \left( \Lambda_0, \mathrm{Cone} (c) \right) \\
%	& = \mathrm{Cone} \left( \mcA_{long} \left( \Lambda_0, \Lambda_i \right) \xrightarrow{\mu^2 \left( -, c \right)} \mcA_{long} \left( \Lambda_0, \Lambda_{i+1} \right) \right),
%	\end{align*}
%	which is acyclic according to Lemma \ref{lemma multiplication by the minimum}
%	Similarly, we have 
%	\[\ker \left( \widetilde{\pi}_{|\mcA_+ \left( \mathrm{Cone} (c), \Lambda_0 \right)} \right) = \mathrm{Cone} \left( \mcA_{long} \left( \Lambda_{i+1}, \Lambda_0 \right) \xrightarrow{\mu^2 \left( c, - \right)} \mcA_{long} \left( \Lambda_i, \Lambda_0 \right) \right), \]
%	which is also acyclic according to Lemma \ref{lemma multiplication by the minimum}
%	
%	Now, let $c \in \mcR \left( \Lambda_i, \Lambda_{i+1} \right) \cap W_+$ and $c' \in \mcR \left( \Lambda_j, \Lambda_{j+1} \right) \cap W_+$. Then 
%	\begin{align*}
%	\ker \left( \widetilde{\pi}_{|\mcA_+ \left( \mathrm{Cone} (c), \mathrm{Cone} (c') \right)} \right) & = \mcA_{long} \left( \mathrm{Cone} (c), \mathrm{Cone} (c') \right) \\
%	& \mkern -150mu = \mathrm{Cone} \left( \mcA_{long} \left( \Lambda_{i+1}, \mathrm{Cone} (c') \right) \xrightarrow{\mu^2 \left( c, - \right)} \mcA_{long} \left( \Lambda_i, \mathrm{Cone} (c') \right) \right) .
%	\end{align*}
%	Besides, 
%	\[\left\{
%	\begin{array}{cll}
%	\mcA_{long} \left( \Lambda_{i+1}, \mathrm{Cone} (c') \right) & = & \mathrm{Cone} \left( \mcA_{long} \left( \Lambda_{i+1}, \Lambda_j \right) \xrightarrow{\mu^2 \left( -, c' \right)} \mcA_{long} \left( \Lambda_{i+1}, \Lambda_{j+1} \right) \right) \\
%	\mcA_{long} \left( \Lambda_i, \mathrm{Cone} (c') \right) & = & \mathrm{Cone} \left( \mcA_{long} \left( \Lambda_i, \Lambda_j \right) \xrightarrow{\mu^2 \left( -, c' \right)} \mcA_{long} \left( \Lambda_i, \Lambda_{j+1} \right) \right)
%	\end{array}
%	\right. . \]
%	Now observe that we have the following commutative diagram of chain complexes
%	\[\begin{tikzcd}
%	A^{i+1, j} \ar[r, "{\mu^2 (-, c')}"] \ar[d, "{\mu^2 (c, -)}"] & A^{i+1, j+1}  \ar[d, "{\mu^2 (c, -)}"] \ar[r] & B^{i+1} \ar[r] \ar[d, "{\mu^2 (c, -)}"] & A^{i+1, j} \ar[r, "{\mu^2 (-, c')}"] \ar[d, "{\mu^2 (c, -)}"] & A^{i+1, j+1}  \ar[d, "{\mu^2 (c, -)}"] \\
%	A^{i,j} \ar[r, "{\mu^2 (-, c')}"] & A^{i,j+1} \ar[r] & B^i \ar[r] & A^{i,j} \ar[r, "{\mu^2 (-, c')}"] & A^{i,j+1}  
%	\end{tikzcd} \]
%	where 
%	\[A^{p,q} = \mcA_{long} \left( \Lambda_p, \Lambda_q \right) \text{ and } B^p = \mcA_{long} \left( \Lambda_p, \mathrm{Cone} (c') \right) . \]
%	Since the maps $\mu^2 \left( c, - \right) : \mcA_{long} \left( \Lambda_{i+1}, \Lambda_j \right) \to \mcA_{long} \left( \Lambda_i, \Lambda_j \right)$ and $\mu^2 \left( c, - \right) : \mcA_{long} \left( \Lambda_{i+1}, \Lambda_{j+1} \right) \to \mcA_{long} \left( \Lambda_i, \Lambda_{j+1} \right)$ are quasi-isomorphisms by Lemma \ref{lemma multiplication by the minimum}, we deduce from the five Lemma that the remaining vertical map $\mu^2 \left( c, - \right) : \mcA_{long} \left( \Lambda_{i+1}, \mathrm{Cone} (c') \right) \to \mcA_{long} \left( \Lambda_i, \mathrm{Cone} (c') \right)$ is also a quasi-isomorphism, and thus that $\ker \left( \widetilde{\pi}_{|\mcA_+ \left( \mathrm{Cone} (c), \mathrm{Cone} (c') \right)} \right)$ is acyclic. This concludes the proof.
%	
%\end{proof}

We denote by $\mcA_+$, $\mcA_{++}$, $\mcA_0$ the $A_{\infty}$-categories associated to $\Lambda$ and $\varepsilon_L$ in Definition \ref{definition several categories}. We now associate an $A_{\infty}$-category to $L$.

\begin{defin}
	
	Let 
	\[\mathbf{L} := \left( L_n \right)_{n \in \mathbf{Z}}. \]
	We denote by $\mcO$ the $A_{\infty}$-category defined as follows:
	\begin{enumerate}
		
		\item the objects of $\mcO$ are the Lagrangians $L_n$, $n \in \mathbf{Z}$, 
		
		\item the space of morphisms from $L_i$ to $L_j$ is either generated by $L_i \cap L_j$ if $i<j$, or $\mathbf{F}$ if $i=j$, or $0$ if $i>j$ ; the bigrading of an intersection point $c \in \mcO \left( \Lambda^i, \Lambda^j \right)$ corresponding to $q_0 \in \mathrm{Crit} \, h_0$ is $\left( 2 \left( j-i \right) + \mathrm{ind} \left( q_0 \right) \right)$, and 
		
		\item the operations are such that $e_{L_n} \in \mcO \left( L_n, L_n \right)$ is a strict unit, and for every sequence of integers $i_0 < \dots < i_d$, for every sequence of intersection points 
		\[\left( x_1, \dots, x_d \right) \in \left( L_{i_0} \cap L_{i_1} \right) \times \dots \times \left( L_{i_{d-1}} \cap L_{i_d} \right) \]
		we have 
		\[\mu_{\mcO} \left( x_1, \dots, x_d \right) = \sum \limits_{x_0 \in L_{i_0} \cap L_{i_d}} \# \mcM_{x_0, x_d \dots x_1} \left( \mathbf{L}, j \right) x_0 \]
		(see Definition \ref{definition moduli spaces for Lagrangians}).
		Besides, let $W_L$ be the set made of the morphisms $u^n \in \mcO \left( L_n, L_{n+1} \right)$ corresponding to the minimum of $\left( H_{n+1} - H_n \right)$ for $n \in \mathbf{N}$.
		We define
		\[CF^* \left( L \right) := \mathrm{End}_{\mcO \left[ W_L^{-1} \right]} \left( L \right) . \]
		
	\end{enumerate} 	
	
\end{defin}

%\begin{defin}
%	
%	Let $\mcO_{\Lambda}$ be the $A_{\infty}$-category such that
%	\begin{enumerate}
%		
%		\item the set of objects of $\mcO_{\Lambda}$ is $\{ \Lambda_n \mid n \in \mathbf{N} \}$,
%		
%		\item the space of morphisms from $\Lambda_i$ to $\Lambda_j$ is either $\langle \mathrm{graph} \left( dh_i \right) \cap \mathrm{graph} \left( dh_j \right) \rangle$ if $i<j$, or $\mathbf{k}$ if $i=j$, or $0$ if $i>j$, and
%		
%		\item the operations count punctured pseudo-holomorphic discs in $T^* \Lambda$ with boundary on $\bigcup\limits_{n \in \mathbf{N}} \mathrm{graph} \left( dh_n \right)$ and asymptotic to intersection points at punctures. 
%		
%	\end{enumerate}
%	Besides, let $W_{\Lambda}$ be the set made of the morphisms $x^n \in \mcO_{\Lambda} \left( \Lambda_n, \Lambda_{n+1} \right)$ corresponding to the minimum of $\left( h_{n+1} - h_n \right)$ for $n \in \mathbf{N}$.
%	We define
%	\[CF^* \left( \Lambda \right) := \mathrm{End}_{\mcO_{\Lambda} \left[ W_{\Lambda}^{-1} \right]} \left( \Lambda \right) . \]
%	
%\end{defin}

There are natural $A_{\infty}$-functors $\psi : \mcO \to \mcA_{++}$ (see \cite{EL21} section 5), $\iota : \mcA_{++} \to \mcA_+$ (the inclusion) and $\pi : \mcA_+ \to \mcA_0$ (the projection).  
The composition $\phi = \pi \circ \iota \circ \psi : \mcO \to \mcA_0$ sends $W_L$ to $W_0$, and thus it induces an $A_{\infty}$-map $\widetilde{\phi} : CF^* \left( L \right) \to LA_0^* \left( \Lambda \right)$.

\begin{defin}\label{definition relative cohomology} 
	
	The Floer complex of $L$ relative to its boundary $\Lambda$ is the non unital $A_{\infty}$-algebra
	\[CF^* \left( L, \Lambda \right) := \mathrm{Cone} \left( CF^* \left( L \right) \xrightarrow{\widetilde{\phi}} LA_0^* \left( \Lambda \right) \right) \]
	(see Definition \ref{definition cone of an algebra map}). 
	
\end{defin}

\section{Results}

Recall that we are considering $A_{\infty}$ functors $\psi : \mcO \to \mcA_{++}$ (as in \cite{EL21} section 5) and $\iota : \mcA_{++} \to \mcA_+$ (the inclusion). Moreover, the composition $\iota \circ \psi : \mcO \to \mcA_+$ sends $W_L$ to $W_+$.

\begin{thm}\label{thm relation Lagrangians Legendrians}
	(Part of Theorem 63 in \cite{EL21})
	
	If $HW^* \left( L \right) = 0$, then the $A_{\infty}$-map
	\[\widetilde{\iota \circ \psi} : CF^* \left( L \right) \to LA_+^* \left( \Lambda \right) \]
	induced by $\iota \circ \psi$ is a quasi-isomorphism.  
	
\end{thm}

\begin{proof}
	
	On the objects, $\psi \left( L_n \right) = \Lambda_n$ and, on the morphisms, $\psi$ is defined using the exact same count of pseudo-holomorphic curves than in \cite{EL21} Theorem 63 (the corresponding $A_{\infty}$-map is denoted $\mathfrak{e}$ there). In \cite{EL21} Theorem 63, the authors prove that for every $i < j$,
	\[\mathrm{Cone} \left( \mcO \left( L_i, L_j \right) \xrightarrow{\psi} \mcA_{++} \left( \Lambda_i, \Lambda_j \right) \right)^{\#} \simeq CW^* \left( L_i, \widehat{L_j} \right) \]
	where $\widehat{L_j}$ is a negative wrapping of $L_j$ across $L_i$.
	By hypothesis, $CW^* \left( L \right)$ is acyclic, which implies that $\psi^1$ is a quasi-isomorphism. Thus, $\psi$ is a quasi-equivalence, and since it sends $W_L$ into $W_+^{dir}$, the induced functor $\widetilde{\psi} : \mcO \left[ W_L^{-1} \right] \to \mcA_{++} \left[ \left( W_+^{dir} \right)^{-1} \right]$ is also a quasi-equivalence (see Lemma 2.4 in \cite{GPS19}). This concludes the proof according to Lemma \ref{lemma directed and non-directed positive augmentation categories}.
	%	If $i < j$, then  
	%	\[\mathrm{Cone} \left( L_i \xrightarrow{\psi^1} L_j \right)^{\mathrm{dual}} = \mathrm{Cth}_+ \left( L_i, L_j \right) . \]
	%	Then, let $\widehat{L_j}$ be a negative wrapping of $L_j$ across $L_i$. By the invariance properties of $\mathrm{Cth}_+$ (see \cite{Leg21}) and the SFT description of $CW^*$ we have 
	%	\[\mathrm{Cth}_+ \left( L_i, L_j \right) \simeq \mathrm{Cth}_+ \left( L_i, \widehat{L_j} \right) \simeq CW^* \left( L_i, \widehat{L_j} \right) . \]
	%	By hypothesis, $CW^* \left( L \right)$ is acyclic, which implies that $\psi^1$ is a quasi-isomorphism. Thus, $\psi$ is a quasi-equivalence, and since it sends $W_+$ into $W_L$, the induced functor $\mcO \left[ W_L_{-1} \right] \to \mcA_+ \left[ W_+^{-1} \right]$ is also a quasi-equivalence (see Lemma 9.2 in \cite{GPS18b}).
	
\end{proof}

\begin{thm}
	(Part of Theorem 63 in \cite{EL21})
	
	If $HW^* \left( L \right) = 0$, then there is a quasi-isomorphism of $A_{\infty}$-algebras
	\[\mathbf{F} \oplus CF^* \left( L, \Lambda \right) \xrightarrow{\sim} LA^* \left( \Lambda \right) . \] 
	
\end{thm}

\begin{proof}
	
%	First recall that there is a quasi-isomorphism
%	\[E \left( CE_{-*} \left( \Lambda \right) \right) \simeq LA^* \left( \Lambda \right) = \mathbf{F} \oplus \overline{LA^*} \left( \Lambda \right) \]
%	(see section \ref{section Chekanov-Eliashberg algebra}).
	First recall that the projection to the space of short Reeb chords induces an $A_{\infty}$-functor $\pi : \mcA_+ \to \mcA_0$ which sends $W_+$ to $W_0$, and Proposition \ref{prop Lagrangian algebra as a cone} gives
	\[\overline{LA^*} \left( \Lambda \right) \simeq \mathrm{Cone} \left( LA_+^* \left( \Lambda \right) \xrightarrow{\widetilde{\pi}} LA_0^* \left( \Lambda \right) \right) . \] 
	Then, recall that the composition $\phi = \pi \circ \iota \circ \psi : \mcO \to \mcA_0$ sends $W_L$ to $W_0$, and thus it induces an $A_{\infty}$-map $\widetilde{\phi} : CF^* \left( L \right) \to LA_0^* \left( \Lambda \right)$. 
	Now observe that we have the following commutative diagram
	\[\begin{tikzcd}
	CF^* \left( L \right) \ar[r, "\widetilde{\iota \circ \psi}"] \ar[d, "\widetilde{\phi}"] & LA_+^* \left( \Lambda, \varepsilon_L \right) \ar[d, "\widetilde{\pi}"] \\
	LA_0^* \left( \Lambda, \varepsilon_L \right) \ar[r, equal] &  LA_0^* \left( \Lambda, \varepsilon_L \right) .
	\end{tikzcd} \]
	The top horizontal arrow is a quasi-isomorphism by Theorem \ref{thm relation Lagrangians Legendrians}. According to Proposition \ref{prop invariance cone of an algebra map}, we get a quasi-isomorphism of non unital $A_{\infty}$-algebras  
	\[CF^* \left( L, \Lambda \right) \xrightarrow{\sim} \overline{LA^*} \left( \Lambda \right). \]
	This concludes the proof because 
	\[LA^* \left( \Lambda \right) = \mathbf{F} \oplus \overline{LA^*} \left( \Lambda \right). \]
	
\end{proof}


\begin{thm}\label{thm dga with coefficients in chains of based loop space}
	(Theorem 51 in \cite{EL21})
	
	If $\Lambda$ is simply connected, then 
	\[E \left( CE_{-*}^+ \left( \Lambda \right) \right) \simeq LA_+^* \left( \Lambda \right) . \]
	
\end{thm}

\begin{proof}[Idea of proof]
	
	Assume that we can choose the copies to be parallel. In \cite{EL21} section 3.5, the authors define a quasi-isomorphism $\phi : CE_{-*}^+ \left( \Lambda\right) \to CE_{-*}^{\parallel} \left( \Lambda \right)$. Applying first bar and then graded dual, we get a quasi-isomorphism $B \left( CE_{-*}^{\parallel} \left( \Lambda \right) \right)^{\#} \to B \left( CE_{-*}^+ \left( \Lambda \right) \right)^{\#}$. Besides, recall that 
	\[CE_{-*}^{\parallel} \left( \Lambda \right) = \Omega LC_*^{\parallel} \left( \Lambda \right). \]
	There is a natural quasi-isomorphism $B \left( \Omega LC_*^{\parallel} \left( \Lambda \right) \right) \to LC_*^{\parallel} \left( \Lambda \right)$ (see section 2.2.2 in \cite{EL21}), which induces a quasi-isomorphism $LA^*_{\parallel} \left( \Lambda \right) \to B \left( \Omega LC_*^{\parallel} \left( \Lambda \right) \right)^{\#}$. As a result, we get a quasi-isomorphism 
	\[LA^*_{\parallel} \left( \Lambda \right) \to B \left( CE_{-*} \left( \Lambda \right) \right)^{\#} . \] 
	
	Now going back to the case where the copies are not parallel, we should still be able to define an $A_{\infty}$-functor $\Phi : \mcA_+ \to B \left( CE_{-*} \left( \Lambda, C_{-*} \left( \Omega \Lambda \right) \right) \right)^{\#}$ which mimic the map we just described. This functor should look like this. Take sequences 
	\[\left\{
	\begin{array}{ccl}
	\left( c_0, \dots, c_{d-1} \right) & \in & \mcR \left( \Lambda_{n_0}, \Lambda_{n_1} \right) \times \dots \times \mcR \left( \Lambda_{n_{d-1}}, \Lambda_{n_d} \right) \\
	\left( x_0, \dots, x_{r-1} \right) & \in & CE_{-*}^+ \left( \Lambda \right)^{r}
	\end{array}
	\right. \]
	such that none of the Reeb chords $c_i$ correspond to the minimum of the Morse function $f_1$, and each $x_i$ is a word in elements of $C_{-*} \left( \Omega \Lambda \right) \cup \mcR \left( \Lambda \right)$.
	If $r$ is positive, then 
	\[\langle \Phi \left( c_0, \dots, c_{d-1} \right), s x_0 \otimes \dots \otimes s x_{r-1} \rangle = 0 . \]
	Assume now that $r=0$. Let $\left( \mathbf{y}_1, \dots, \mathbf{y}_p \right)$ be the family of short Reeb chords appearing in $c_0 \cdots c_{d-1}$.
	Then 
	\[	\langle \Phi \left( c_0, \dots, c_{d-1} \right), s x_0 \rangle = \prod_{i=1}^{p} \vert \mcT \left( \sigma_i, \mathbf{y}_i \right) \vert \]
	(the moduli spaces $\mcT \left( \sigma_i, \mathbf{y}_i \right)$ are defined in \cite{EL21} section 3.5) if $x_0$ is obtained from $c_0 \cdots c_{d-1}$ by replacing each $\mathbf{y}_i$ by $\sigma_i$, and $0$ otherwise. 
	
	%	For any positive integer $r$, let 
	%	\[ I_r := \{ \mathbf{i} = \left( i_0, \dots, i_r \right) \in \mathbf{N}^{r+1} \mid 0=i_0 < \dots < i_r=d \} . \] 
	%	Take sequences 
	%	\[\left\{
	%	\begin{array}{ccl}
	%	\left( c_0, \dots, c_{d-1} \right) & \in & \mcA \left( \Lambda_{n_0}, \Lambda_{n_1} \right) \times \dots \times \mcA \left( \Lambda_{n_{d-1}}, \Lambda_{n_d} \right) \\
	%	\left( x_0, \dots, x_{r-1} \right) & \in & CE_{-*} \left( \Lambda, C_{-*} \left( \Omega \Lambda \right) \right)^{r}
	%	\end{array}
	%	\right. . \]
	%	Then 
	%	\[\langle \Phi \left( c_0, \dots, c_{d-1} \right), s x_0 \otimes \dots \otimes s x_{r-1}   \rangle = \sum\limits_{\mathbf{i} \in I_r} \prod_{j=0}^{r-1} \mu \left( \mathbf{i}, j \right) \]
	%	where $\mu \left( \mathbf{i}, j \right) \in \mathbf{k}$ is defined as follows. Let $\left( \mathbf{y}_1, \dots, \mathbf{y}_p \right)$ be the family of short Reeb chords appearing in $c_{i_j} \dots c_{i_{j+1}-1}$. Then 
	%	\[\mu \left( \mathbf{i}, j \right) = \prod_{k=1}^{p} \vert \mcT \left( \sigma_k, \mathbf{y}_k \right) \vert \]
	%	if $x_j$ is obtained from $c_{i_j} \dots c_{i_{j+1}-1}$ by replacing each $\mathbf{y}_k$ by $\sigma_k \in C_{-*} \left( \Omega \Lambda \right)$, and $0$ otherwise.
	
	It remains to show that $\Phi$ sends $W_+$ to the unit (this should follow from Lemma 38 in \cite{EL21}), and that the induced functor $\widetilde{\Phi} : \mcA_+ \left[ W_+^{-1} \right] \to B \left( CE_{-*}^+ \left( \Lambda \right) \right)^{\#} \left[ \mathbf{1}^{-1} \right]$ is a quasi-equivalence. 
	
\end{proof}

%\begin{thm}
%	
%	If $\Lambda$ is simply connected, then
%	\[E \left( CE_{-*}^+ \left( \Lambda \right) \right) \simeq CF^* \left( L \right) . \] 
%	
%\end{thm}
%
%\begin{proof}
%	
%	This follows from Theorems \ref{thm dga with coefficients in chains of based loop space} and \ref{thm relation Lagrangians Legendrians}.
%	
%\end{proof}

%\begin{rmk}
%	
%	It follows from Remark \ref{relation with augmentation categories} and Theorem \ref{thm relation Lagrangians Legendrians} that, if $HW^* \left( L \right) = 0$, then we should have a quasi-isomorphism
%	\[\mathrm{End}_{Aug_+} \left( \Lambda, \varepsilon_L \right) \simeq CF^* \left( L \right) .  \]  
%	
%\end{rmk}	

==> Extended_algebra/extended_algebra.tex <==
% !TeX spellcheck = en_US
\section{Extended Legendrian $A_{\infty}$-algebra}\label{subsection positive augmentation category}

In this appendix, we study the endomorphism $A_{\infty}$-algebra $LA_+^* \left( \Lambda \right)$ of an augmentation $\varepsilon : CE_{-*} \left( \Lambda \right) \to \mathbf{F}$ in the positive augmentation category $\mcA ug_+ \left( \Lambda \right)$ defined by Chantraine in \cite{Cha19} (it was first introduced by Ng, Rutherford, Shende, Sivek and Zaslow in \cite{NRS+20} for Legendrians in $\mathbf{R}^3$).
The goal is to prove Proposition \ref{prop Lagrangian algebra as a cone}, which shows that there is a quasi-isomorphism of non-unital $A_{\infty}$-algebras between $\overline{LA^* \left( \Lambda \right)}$ (which is the endomorphism algebra of $\varepsilon$ in the augmentation category $\mcA ug_- \left( \Lambda \right)$ defined in \cite{BC14}) and the cone of an $A_{\infty}$-map from $LA_+^* \left( \Lambda \right)$ to some $A_{\infty}$-algebra $LA_0^* \left( \Lambda \right)$ generated by Morse type generators.

\subsection{Setting}

Let $(V, \xi)$ be a contact manifold of dimension $(2n+1)$ equipped with a hypertight contact form $\alpha$, and let $\Lambda$ be a connected compact Legendrian submanifold in $\left( V, \xi \right)$ which is chord generic with respect to $\alpha$ (see section \ref{subsection Legendrian invariants}).
In the following we fix an augmentation $\varepsilon : CE_{-*} \left( \Lambda \right) \to \mathbf{F}$. 

Choose a positive Morse function $f_1 : \Lambda \to \mathbf{R}$ with a unique minimum.
We denote by $\mcU$ a small open neighborhood of $f_1$ in $C^{\infty} \left( \Lambda \right)$ with the following property: for every $f$ in $\mcU$, $f$ is positive, Morse, and its critical points and gradient trajectories are in bijection with those of $f_1$. 
Then we choose a family $\left( f_n \right)_{n \geq 2}$ of functions in $\mcU$.
We also choose a decreasing sequence $\left( \delta_k \right)_{k \geq 1}$ of small enough positive numbers so that the family
\[h_n = \sum_{k=1}^{n} \delta_k f_k, \quad n \in \mathbf{N}, \]
has the following property: for every $i<j$, $\left( h_j - h_i \right)$ lies in the cone over $\mcU$ (this can be easily achieved by induction on $n$).
Finally, we let $\Lambda_n \subset V$ be the Legendrian corresponding to the one-jet of $h_n$ in a Weinstein neighborhood of $\Lambda = \Lambda_0$. 
Observe that if the numbers $\delta_k$ are small enough, the Chekanov-Eliashberg DG-algebra of $\Lambda_n$ is naturally identified with $CE_{-*} \left( \Lambda \right)$ for every $n$. In particular, $\varepsilon = \varepsilon_0$ induces an augmentation $\varepsilon_n : CE_{-*} \left( \Lambda_n \right) \to \mathbf{F}$ for every $n$. 

\begin{rmk}
	
	Let $\eta$ be the length of the smallest Reeb chord of $\Lambda$. The set $\mcR \left( \Lambda_i, \Lambda_j \right)$ of Reeb chords starting on $\Lambda_i$ and ending on $\Lambda_j$ splits as 
	\[\mcR \left( \Lambda_i, \Lambda_j \right) = \mcR_{long} \left( \Lambda_i, \Lambda_j \right) \sqcup \mcR_{short} \left( \Lambda_i, \Lambda_j \right), \]
	where $\mcR_{long} \left( \Lambda_i, \Lambda_j \right)$ is the set of chords with length greater than $\eta / 2$ (and $\mcR_{short} \left( \Lambda_i, \Lambda_j \right)$ is the complementary set). In the following, we choose the numbers $\delta_k$ small enough so that the maximum of $h_n$ is very small compare to $\eta$. In particular, the set $\mcR_{short} \left( \Lambda_i, \Lambda_j \right)$ is empty when $i \geq j$, and it is in bijection with $\mathrm{Crit} \left( h_j - h_i \right)$ when $i < j$. 
	
\end{rmk}

\subsection{Some $A_{\infty}$-categories and $A_{\infty}$-algebras}

In the following, we fix a regular almost complex structure $J$ on $\xi$ (see subsection \ref{subsection moduli spaces}).  
We define three $A_{\infty}$-categories $\mcA_{\triangle}$, for $\triangle \in \{ ++, +, 0 \}$.
$\mcA_{++}$ corresponds to the directed $A_{\infty}$-category used in \cite{Cha19} subsection 3.3 in order to define the endomorphism algebra of $\varepsilon$ in $\mcA ug_+ \left( \Lambda \right)$, $\mcA_+$ is a non-directed version of $\mcA_{++}$, and $\mcA_0$ is an $A_{\infty}$-category whose spaces of morphisms are generated by short Reeb chords.

\begin{defin}\label{definition several categories}
	
	Let
	\[\mathbf{\Lambda} := \bigsqcup_{n \in \mathbf{N}} \Lambda_n.  \]
	We consider the $A_{\infty}$-categories $\mcA_{\triangle}$, $\triangle \in \{ ++, +, 0 \}$, defined as follows:
	\begin{enumerate}
		
		\item the set of objects of $\mcA_{\triangle}$ is $\{ \Lambda_n \mid n \in \mathbf{N} \}$,
		
		\item the space of morphisms from $\Lambda_i$ to $\Lambda_j$ is
		\[\mcA_{\triangle} \left( \Lambda_i, \Lambda_j \right) = \left\{
		\begin{array}{ll}
		\langle \mcR \left( \Lambda_i, \Lambda_j \right) \rangle & \text{if } \triangle \in \{ +, ++ \} \\
		\langle \mcR_{short} \left( \Lambda_i, \Lambda_j \right) \rangle & \text{if } \triangle = 0 
		\end{array}
		\right. \]
		if $i < j$,
		\[\mcA_{\triangle} \left( \Lambda_i, \Lambda_i \right) = \left\{
		\begin{array}{ll}
		\mathbf{F} & \text{if } \triangle \in \{ ++, 0 \} \\
		\mathbf{F} \oplus \langle \mcR \left( \Lambda_i, \Lambda_i \right) \rangle & \text{if } \triangle = + ,
		\end{array}
		\right. \] 
		and $\mcA_{\triangle} \left( \Lambda_i, \Lambda_j \right) = 0$ if $i > j$. 
		
		\item the operations are such that $e_{\Lambda_n} \in \mcA_{\triangle} \left( \Lambda_n, \Lambda_n \right)$ is a strict unit, and for every sequence of generators 
		\[\left( x_1, \dots, x_d \right) \in \mcA_{\triangle} \left( \Lambda_{i_0}, \Lambda_{i_1} \right) \times \dots \times \mcA_{\triangle} \left( \Lambda_{i_{d-1}}, \Lambda_{i_d} \right), \]
		we have 
		\begin{align*}
		\mu_{\mcA_{\triangle}} & \left( x_1, \dots, x_d \right) \\ 
		& = \sum \limits_{\substack{ a, \boldsymbol{\gamma_0}, \dots, \boldsymbol{\gamma_d} }} \# \mcM_{a, \boldsymbol{\gamma_d} x_d \boldsymbol{\gamma_{d-1}} x_{d-1} \dots x_1 \boldsymbol{\gamma_0}} \left( \mathbf{R} \times \mathbf{\Lambda}, J \right) \varepsilon_{i_0} \left( \boldsymbol{\gamma_0} \right) \dots \varepsilon_{i_d} \left( \boldsymbol{\gamma_d} \right)  a ,
		\end{align*}
		where in the sum, $a$ is a generator of $\mcA_{\triangle} \left( \Lambda_{i_0}, \Lambda_{i_d} \right)$ and $\boldsymbol{\gamma_j}$ is a word of Reeb chords in $\mcR \left( \Lambda_{i_j}, \Lambda_{i_j} \right)$
		(see Definition \ref{definition moduli spaces} for the moduli spaces).
		
	\end{enumerate}
	Moreover, we let $W_{\triangle}$ be the set made of the generators $c_n \in \mcA_{\triangle} \left( \Lambda_n, \Lambda_{n+1} \right)$ corresponding to the minimum of $\left( h_{n+1} - h_n \right)$ for $n \in \mathbf{N}$.
	We define
	\[LA_{\triangle}^* \left( \Lambda \right) := \mathrm{End}_{\mcA_{\triangle} \left[ W_{\triangle}^{-1} \right]} \left( \Lambda \right) . \]
	
\end{defin}

\begin{lemma}\label{lemma multiplication by the minimum in the different versions}
	
	For every integer $j$, for every $\triangle \in \{ ++, +, 0 \}$ the morphism $c_j \in \mcA_{\triangle} \left( \Lambda_j, \Lambda_{j+1} \right) \cap W_{\triangle}$ satisfies the following. For every $i < j < k$, the chain maps
	\[\left\{
	\begin{array}{ccccl}
	\mu_{\mcA_{\triangle}}^2 \left( - , c_j \right) & : & \mcA_{\triangle} \left( \Lambda_i , \Lambda_j \right) & \to & \mcA_{\triangle} \left( \Lambda_i , \Lambda_{j+1} \right) \\
	\mu_{\mcA_{\triangle}}^2 \left( c_j , - \right) & : & \mcA_{\triangle} \left( \Lambda_{j+1}, \Lambda_{k+1} \right) & \to & \mcA_{\triangle} \left( \Lambda_j, \Lambda_{k+1} \right)
	\end{array}
	\right. \]
	are quasi-isomorphisms. 
	Moreover, if we denote by $\mcA_{long} \left( \Lambda_m, \Lambda_n \right)$ the subcomplex of $\mcA_+ \left( \Lambda_m, \Lambda_n \right)$ generated by $\mcR_{long} \left( \Lambda_m, \Lambda_n \right)$, then the induced chain maps 
	\[\left\{
	\begin{array}{ccccl}
	\mu_{\mcA_+}^2 \left( - , c_j \right) & : & \mcA_{long} \left( \Lambda_i , \Lambda_j \right) & \to & \mcA_{long} \left( \Lambda_i , \Lambda_{j+1} \right) \\
	\mu_{\mcA_+}^2 \left( c_j , - \right) & : & \mcA_{long} \left( \Lambda_{j+1}, \Lambda_{k+1} \right) & \to & \mcA_{long} \left( \Lambda_j, \Lambda_{k+1} \right)
	\end{array}
	\right. \]
	also are quasi-isomorphisms. 
	
\end{lemma}

\begin{proof}
	
	When the contact manifold is $V = \mathbf{R} \times P$, the result follows from the main analytic theorem of \cite{EES09} (Theorem 3.6). Indeed, this result implies that (when the perturbation functions $h_n$ are small enough) the 3-punctured pseudo-holomorphic discs with boundary on $\mathbf{R} \times \bigsqcup_n \Lambda_n$, asymptotic to $c_j$ at one of their punctures, correspond to trivial cylinders with boundary on $\mathbf{R} \times \Lambda$.
	
	The general case is part of a work in progress of Chantraine, Dimitroglou-Rizell and Ghiggini. 
	
\end{proof}

%\begin{defin}\label{definition positive augmentation category}
%	
%	Let
%	\[\mathbf{\Lambda} := \bigsqcup_{n \in \mathbf{N}} \Lambda_n.  \]
%	We consider the $A_{\infty}$-category $\mcA_+$ defined as follows:
%	\begin{enumerate}
%		
%		\item the set of objects of $\mcA_+$ is $\{ \Lambda_n \mid n \in \mathbf{N} \}$,
%		
%		\item the space of morphisms from $\Lambda_i$ to $\Lambda_j$ is either $\langle \mcR \left( \Lambda_i, \Lambda_j \right) \rangle$ if $i \ne j$ ($\langle E \rangle$ denotes the vector space generated by the set $E$), or $\mathbf{F} \oplus \langle \mcR \left( \Lambda_i \right) \rangle$ if $i=j$, and
%		
%		\item the operations are such that $e_{\Lambda_n} \in \mcA_+ \left( \Lambda_n, \Lambda_n \right)$ is a strict unit, and for every sequence of Reeb chords 
%		\[\left( x_1, \dots, x_d \right) \in \mcR \left( \Lambda_{i_0}, \Lambda_{i_1} \right) \times \dots \times \mcR \left( \Lambda_{i_{d-1}}, \Lambda_{i_d} \right), \]
%		we have 
%		\begin{align*}
%		\mu_{\mcA_+} & \left( x_1, \dots, x_d \right) \\ 
%		& = \sum \limits_{\substack{ a \in \mcR \left( \Lambda^{i_0}, \Lambda^{i_d} \right) \\ \boldsymbol{\gamma_0}, \dots, \boldsymbol{\gamma_d} }} \# \mcM_{a, \boldsymbol{\gamma_d} x_d \boldsymbol{\gamma_{d-1}} x_{d-1} \dots x_1 \boldsymbol{\gamma_0}} \left( \mathbf{R} \times \mathbf{\Lambda} \right) \varepsilon_{i_0} \left( \boldsymbol{\gamma_0} \right) \dots \varepsilon_{i_d} \left( \boldsymbol{\gamma_d} \right)  a 
%		\end{align*}
%		where in the sum, $\boldsymbol{\gamma_j}$ is a word of Reeb chords in $\mcR \left( \Lambda_{i_j} \right)$
%		(see Definition \ref{definition moduli spaces} for the moduli spaces).
%		
%	\end{enumerate}
%	Besides, let $W_+$ be the set made of the morphisms $c_n \in \mcR_{short} \left( \Lambda_n, \Lambda_{n+1} \right)$ corresponding to the minimum of $\left( h_{n+1} - h_n \right)$ for $n \in \mathbf{N}$.
%	We define
%	\[LA_+^* \left( \Lambda \right) := \mathrm{End}_{\mcA_+ \left[ W_+^{-1} \right]} \left( \Lambda \right) . \]
%	
%\end{defin}
%
%\begin{rmk}
%	
%	In subsection \ref{subsection Chekanov-Eliashberg algebra}, we defined a Legendrian $A_{\infty}$-algebra $LA^* \left( \Lambda \right)$ associated to the Legendrian $\Lambda$ and the augmentation $\varepsilon$. We have 
%	\[LA^* \left( \Lambda \right) = \mathrm{End}_{\mcA_+} \left( \Lambda \right) . \]
%	
%\end{rmk}
%
%\begin{lemma}\label{lemma multiplication by the minimum}
%	
%	For every integer $j$, the morphism $c_j \in \mcA_+ \left( \Lambda_j, \Lambda_{j+1} \right) \cap W_+$ satisfies the following. For every $i < j < k$, the chain maps
%	\[\left\{
%	\begin{array}{ccccl}
%	\mu_{\mcA_+}^2 \left( - , c_j \right) & : & \mcA_+ \left( \Lambda_i , \Lambda_j \right) & \to & \mcA_+ \left( \Lambda_i , \Lambda_{j+1} \right) \\
%	\mu_{\mcA_+}^2 \left( c_j , - \right) & : & \mcA_+ \left( \Lambda_{j+1}, \Lambda_{k+1} \right) & \to & \mcA_+ \left( \Lambda_j, \Lambda_{k+1} \right)
%	\end{array}
%	\right. \]
%	are quasi-isomorphisms. 
%	Moreover, if we denote by $\mcA_{long} \left( \Lambda_m, \Lambda_n \right)$ the subcomplex of $\mcA_+ \left( \Lambda_m, \Lambda_n \right)$ generated by $\mcR_{long} \left( \Lambda_m, \Lambda_n \right)$, then the induced chain maps 
%	\[\left\{
%	\begin{array}{ccccl}
%	\mu_{\mcA_+}^2 \left( - , c_j \right) & : & \mcA_{long} \left( \Lambda_i , \Lambda_j \right) & \to & \mcA_{long} \left( \Lambda_i , \Lambda_{j+1} \right) \\
%	\mu_{\mcA_+}^2 \left( c_j , - \right) & : & \mcA_{long} \left( \Lambda_{j+1}, \Lambda_{k+1} \right) & \to & \mcA_{long} \left( \Lambda_j, \Lambda_{k+1} \right)
%	\end{array}
%	\right. \]
%	also are quasi-isomorphisms. 
%	
%\end{lemma}
%
%\begin{proof}
%	
%	\textcolor{red}{Preuve.}
%	
%\end{proof}
%
%We also define a directed version, following \cite{Cha19} subsection 3.3. 
%
%\begin{defin}\label{definition directed positive augmentation category}
%	
%	We consider the $A_{\infty}$-category $\mcA_{++}$ defined as follows:
%	\begin{enumerate}
%		
%		\item the set of objects of $\mcA_{++}$ is $\{ \Lambda_n \mid n \in \mathbf{N} \}$,
%		
%		\item the space of morphisms from $\Lambda_i$ to $\Lambda_j$ is either $\langle \mcR \left( \Lambda_i, \Lambda_j \right) \rangle$ if $i < j$, or $\mathbf{F}$ if $i=j$, or $0$ if $i>j$, and
%		
%		\item the operations are such that $e_{\Lambda_n} \in \mcA_{++} \left( \Lambda_n, \Lambda_n \right)$ is a strict unit, and for every sequence of integers $i_0 < \dots < i_d$, for every sequence of Reeb chords 
%		\[\left( x_1, \dots, x_d \right) \in \mcR \left( \Lambda_{i_0}, \Lambda_{i_1} \right) \times \dots \times \mcR \left( \Lambda_{i_{d-1}}, \Lambda_{i_d} \right) \]
%		we have 
%		\begin{align*}
%		\mu_{\mcA_{++}} & \left( x_1, \dots, x_d \right) \\ 
%		& = \sum \limits_{\substack{ a \in \mcR \left( \Lambda^{i_0}, \Lambda^{i_d} \right) \\ \boldsymbol{\gamma_0}, \dots, \boldsymbol{\gamma_d} }} \# \mcM_{a, \boldsymbol{\gamma_d} x_d \boldsymbol{\gamma_{d-1}} x_{d-1} \dots x_1 \boldsymbol{\gamma_0}} \left( \mathbf{R} \times \mathbf{\Lambda} \right) \varepsilon_{i_0} \left( \boldsymbol{\gamma_0} \right) \dots \varepsilon_{i_d} \left( \boldsymbol{\gamma_d} \right)  a 
%		\end{align*}
%		where in the sum, $\boldsymbol{\gamma_j}$ is a word of Reeb chords in $\mcR \left( \Lambda_{i_j} \right)$ (see Definition \ref{definition moduli spaces} for the moduli spaces).
%		
%	\end{enumerate}
%	Besides, let $W_{++}$ be the set made of the morphisms $c_n \in \mcA_{++} \left( \Lambda_n, \Lambda_{n+1} \right)$ corresponding to the minimum of $\left( h_{n+1} - h_n \right)$ for $n \in \mathbf{N}$.
%	
%\end{defin}
%
%\begin{rmk}
%	
%	In \cite{Cha19} subsection 3.3, the author defined an $A_{\infty}$-category $\mcA ug_+ \left( \Lambda \right)$. We have 
%	\[\mcA_{++} \left[ \left( W_{++} \right)^{-1} \right] = \mathrm{End}_{\mcA ug_+ \left( \Lambda \right)} \left( \varepsilon \right) . \]
%	
%\end{rmk}
%
%\begin{lemma}\label{lemma multiplication by the minimum in directed version}
%	
%	For every integer $j$, the morphism $c_j \in \mcA_{++} \left( \Lambda_j, \Lambda_{j+1} \right) \cap W_{++}$ satisfies the following. For every $i < j < k$, the chain maps
%	\[\left\{
%	\begin{array}{ccccl}
%	\mu_{\mcA_{++}}^2 \left( - , c_j \right) & : & \mcA_{++} \left( \Lambda_i , \Lambda_j \right) & \to & \mcA_{++} \left( \Lambda_i , \Lambda_{j+1} \right) \\
%	\mu_{\mcA_{++}}^2 \left( c_j , - \right) & : & \mcA_{++} \left( \Lambda_{j+1}, \Lambda_{k+1} \right) & \to & \mcA_{++} \left( \Lambda_j, \Lambda_{k+1} \right)
%	\end{array}
%	\right. \]
%	are quasi-isomorphisms. 
%	
%\end{lemma}
%
%\begin{proof}
%	
%	\textcolor{red}{Preuve.}
%	
%\end{proof}
%
%\begin{defin}\label{definition local category for a Legendrian}
%	
%	We consider the $A_{\infty}$-category $\mcA_0$ defined as follows:
%	\begin{enumerate}
%		
%		\item the set of objects of $\mcA_0$ is $\{ \Lambda_n \mid n \in \mathbf{N} \}$,
%		
%		\item the space of morphisms from $\Lambda_i$ to $\Lambda_j$ is either $\langle \mcR_{short} \left( \Lambda_i, \Lambda_j \right) \rangle$ if $i<j$, or $\mathbf{F}$ if $i=j$, or $0$ if $i>j$, and
%		
%		\item the operations are such that $e_{\Lambda_n} \in \mcA_0 \left( \Lambda_n, \Lambda_n \right)$ is a strict unit, and for every sequence of integers $i_0 < \dots < i_d$, for every sequence of Reeb chords 
%		\[\left( x_1, \dots, x_d \right) \in \mcR_{short} \left( \Lambda_{i_0}, \Lambda_{i_1} \right) \times \dots \times \mcR_{short} \left( \Lambda_{i_{d-1}}, \Lambda_{i_d} \right) \]
%		we have 
%		\[\mu_{\mcA_0} \left( x_1, \dots, x_d \right) = \sum \limits_{a \in \mcR_{short} \left( \Lambda^{i_0}, \Lambda^{i_d} \right)} \# \mcM_{a, x_d \dots x_1} \left( \mathbf{R} \times \mathbf{\Lambda} \right) a \]
%		(see Definition \ref{definition moduli spaces} for the moduli spaces).
%		
%	\end{enumerate}
%	Besides, let $W_0$ be the set made of the morphisms $c_n \in \mcA_0 \left( \Lambda_n, \Lambda_{n+1} \right)$ corresponding to the minimum of $\left( h_{n+1} - h_n \right)$ for $n \in \mathbf{N}$.
%	We define
%	\[LA_0^* \left( \Lambda \right) := \mathrm{End}_{\mcA_0 \left[ W_0^{-1} \right]} \left( \Lambda \right) . \]
%	
%\end{defin}
%
%\begin{lemma}\label{lemma multiplication by the minimum in short version}
%	
%	For every integer $j$, the morphism $c_j \in \mcA_0 \left( \Lambda_j, \Lambda_{j+1} \right) \cap W_0$ satisfies the following. For every $i < j < k$, the chain maps
%	\[\left\{
%	\begin{array}{ccccl}
%	\mu_{\mcA_0}^2 \left( - , c_j \right) & : & \mcA_0 \left( \Lambda_i , \Lambda_j \right) & \to & \mcA_0 \left( \Lambda_i , \Lambda_{j+1} \right) \\
%	\mu_{\mcA_0}^2 \left( c_j , - \right) & : & \mcA_0 \left( \Lambda_{j+1}, \Lambda_{k+1} \right) & \to & \mcA_0 \left( \Lambda_j, \Lambda_{k+1} \right)
%	\end{array}
%	\right. \]
%	are quasi-isomorphisms. 
%	
%\end{lemma}
%
%\begin{proof}
%	
%	\textcolor{red}{Preuve.}
%	
%\end{proof}

\subsection{Relations between $A_{\infty}$-categories and $A_{\infty}$-algebras}

Observe that the inclusion $\iota : \mcA_{++} \to \mcA_+$ defines a strict $A_{\infty}$-functor which sends $W_{++}$ to $W_+$.

%\begin{defin}\label{definition functor from directed to non directed}
%	
%	We consider the strict $A_{\infty}$-functor $\iota : \mcA_{++} \to \mcA_+$ defined as follows:
%	\begin{enumerate}
%		
%		\item on the objects, $\iota \left( \Lambda_n \right) = \Lambda_n$,
%		
%		\item on the morphisms, $\iota$ sends a Reeb chord $c \in \mcR \left( \Lambda_i, \Lambda_j \right)$ to $c$.
%		
%	\end{enumerate}
%	
%\end{defin}

\begin{lemma}\label{lemma directed and non-directed positive augmentation categories}
	
	The $A_{\infty}$-functor
	\[\widetilde{\iota} : \mcA_{++} \left[ W_{++}^{-1} \right] \xrightarrow{\sim} \mcA_+ \left[ W_+^{-1} \right] \]
	induced by $\iota$ (see Definition \ref{definition induced functor between quotients}) is a quasi-equivalence.
	
\end{lemma}

\begin{proof}
	
	Fix an object $Y = \Lambda_m$ in $\mcA_{++}$. We want to prove that the map 
	\[\widetilde{\iota} : \mcA_{++} \left[ W_{++}^{-1} \right] \left( X, Y \right) \to \mcA_+ \left[ W_+ ^{-1} \right] \left( \widetilde{\iota} X, \widetilde{\iota} Y \right) \]
	is a quasi-isomorphism for every object $X$. 
	Our strategy is to apply Proposition \ref{prop quasi-isomorphism between localizations}. We consider the modules $\mcM_{\mcA_+}$, $\mcM_{\mcA_{++}}$ and module maps $t_{\mcA_{++}} : \mcA_{++} \left( -, \Lambda_m \right) \to \mcM_{\mcA_{++}}$, $t_{\mcA_+} : \mcA_+ \left( -, \Lambda_m \right) \to \mcM_{\mcA_+}$ of Definition \ref{definition specific module}. 
	Observe that the diagram of $\mcA_{++}$-modules 
	\[\begin{tikzcd}
	\bigoplus \limits_{n \geq 0} \mcA_{++} \left( -, \Lambda_n \right) \ar[d, "\mathrm{id}"] \ar[r, "\bigoplus \limits_{n \geq 0} t_{c_n}"] & \bigoplus \limits_{n \geq 0} \mcA_{++} \left( -, \Lambda_{n+1} \right) \ar[d, "t_{\iota}"] \\
	\bigoplus \limits_{n \geq 0} \mcA_{++} \left( -, \Lambda_n \right) \ar[r, "t_{\iota}"] & \iota^* \mcM_{\mcA_+}
	\end{tikzcd} \]
	commutes up to the homotopy $h : \bigoplus \limits_{n \geq 0} \mcA_{++} \left( -, \Lambda_n \right) \to \iota^* \mcM_{\mcA_+}$ which is the strict module map sending $x \in \mcA_{++} \left( \Lambda_k, \Lambda_n \right)$ to 
	\[h(x) = sx \in \mcA_+ \left( \Lambda_k, \Lambda_n \right) \left[ 1 \right] \subset \iota^* \mcM_{\mcA_+} \left( \Lambda_k \right) \]
	($s : \mcA_+ \left( \Lambda_k, \Lambda_n \right) \to \mcA_+ \left( \Lambda_k, \Lambda_n \right) \left[ 1 \right]$ is the usual degree $(-1)$ map).
	According to Proposition \ref{prop morphism induced by homotopy}, this induces a closed $\mcA_{++}$-module map $t_0 : \mcM_{\mcA_{++}} \to \iota^* \mcM_{\mcA_+}$. Moreover, the following diagram of $\mcA_{++}$-modules is commutative
	\[\begin{tikzcd}
	\mcA_{++} \left( - , Y \right) \ar[d, "t_{\mcA_{++}}"] \ar[r, "t_{\iota}"] & \iota^* \mcA_+ \left( - , \iota Y  \right) \ar[d, "\iota^* t_{\mcA_+}"] \\
	\mcM_{\mcA_{++}} \ar[r, "t_0"] & \iota^* \mcM_{\mcA_+} .
	\end{tikzcd} \] 
	
	It remains to check the three items of Proposition \ref{prop quasi-isomorphism between localizations}. The first two items are satisfied according to Lemmas \ref{lemma multiplication by the minimum in the different versions} and \ref{lemma second result for specific module}. We now have to prove that $t_0 : \mcM_{\mcA_{++}} \to \iota^* \mcM_{\mcA_+}$ is a quasi-isomorphism. Let $X = \Lambda_k$ be some object in $\mcA_{++}$. Observe that the following diagram of chain complexes is commutative 
	\[\begin{tikzcd}
	\mcM_{\mcA_{++}} \left( \Lambda_k \right) \ar[r, "t_0"] & \iota^* \mcM_{\mcA_+} \left( \Lambda_k \right) = \mcM_{\mcA_+} \left( \Lambda_k \right) \\
	\mcA_{++} \left( \Lambda_k, \Lambda_{k+1} \right) \ar[u, hook] \ar[r, "\iota"] & \mcA_+ \left( \Lambda_k, \Lambda_{k+1} \right) \ar[u, hook] .
	\end{tikzcd} \]
	Each vertical map is a quasi-isomorphism according to Lemma \ref{lemma first result for specific module}, and the bottom horizontal map is the identity map. This implies that $t_0$ is a quasi-isomorphism, which is what we needed to prove.
	
\end{proof}

Observe that the projection $\pi : \mcA_+ \to \mcA_0$ defines a strict $A_{\infty}$-functor which sends $W_+$ to $W_0$. Thus it induces a strict $A_{\infty}$-functor $\widetilde{\pi} : \mcA_+ \left[ W_+^{-1} \right] \to \mcA_0 \left[ W_0^{-1} \right]$ (see Definition \ref{definition induced functor between quotients}). 
Besides, let $\overline{LA^*} \left( \Lambda \right)$ be the augmented ideal of 
\[LA^* \left( \Lambda \right) = \mathrm{End}_{\mcA_+} \left( \Lambda \right) \]
($\overline{LA^*} \left( \Lambda \right)$ is the endomorphism algebra of $\varepsilon$ in the $A_{\infty}$-category $\mcA ug_- \left( \Lambda \right)$ defined in \cite{BC14}, see subsection \ref{subsection Chekanov-Eliashberg algebra}). The inclusion $\overline{LA^*} \left( \Lambda \right) \hookrightarrow \mcA_+ \left( \Lambda, \Lambda \right)$ induces a strict $A_{\infty}$-map $\overline{LA^*} \left( \Lambda \right) \to LA_+^* \left( \Lambda \right)$ whose image is contained in $\ker \left( \widetilde{\pi} \right)$. Since $\ker \left( \widetilde{\pi} \right)$ is an $A_{\infty}$-subalgebra of $\mathrm{Cone} \left( LA_+^* \left( \Lambda \right) \xrightarrow{\widetilde{\pi}} LA_0^* \left( \Lambda \right) \right)$ (see Definition \ref{definition cone of an algebra map}), we get a strict $A_{\infty}$-map 
\[\phi : \overline{LA^*} \left( \Lambda \right) \to \mathrm{Cone} \left( LA_+^* \left( \Lambda \right) \xrightarrow{\widetilde{\pi}} LA_0^* \left( \Lambda \right) \right) . \]

\begin{prop}\label{prop Lagrangian algebra as a cone}
	
	The $A_{\infty}$-map
	\[\phi : \overline{LA^*} \left( \Lambda \right) \to \mathrm{Cone} \left( LA_+^* \left( \Lambda \right) \xrightarrow{\widetilde{\pi}} LA_0^* \left( \Lambda \right) \right) \]
	is a quasi-isomorphism. 
	
\end{prop}

\begin{proof}
	
	We will apply Proposition \ref{prop quasi-isomorphism between localizations} to the $A_{\infty}$-functor $\pi : \mcA_+ \to \mcA_0$ and the object $\Lambda_0 = \Lambda$ of $\mcA_+$. 
	We consider the modules $\mcM_{\mcA_0}$, $\mcM_{\mcA_+}$ and module maps $t_{\mcA_+} : \mcA_+ \left( -, \Lambda \right) \to \mcM_{\mcA_+}$, $t_{\mcA_0} : \mcA_0 \left( -, \Lambda \right) \to \mcM_{\mcA_0}$ of Definition \ref{definition specific module}. 
	Observe that the diagram of $\mcA_+$-modules 
	\[\begin{tikzcd}
	\bigoplus \limits_{n \geq 0} \mcA_+ \left( -, \Lambda_n \right) \ar[d, "\mathrm{id}"] \ar[r, "\bigoplus \limits_{n \geq 0} t_{c_n}"] & \bigoplus \limits_{n \geq 0} \mcA_+ \left( -, \Lambda_{n+1} \right) \ar[d, "t_{\pi}"] \\
	\bigoplus \limits_{n \geq 0} \mcA_+ \left( -, \Lambda_n \right) \ar[r, "t_{\pi}"] & \pi^* \mcM_{\mcA_0}
	\end{tikzcd} \]
	commutes up to the homotopy $h : \bigoplus \limits_{n \geq 0} \mcA_+ \left( -, \Lambda_n \right) \to \pi^* \mcM_{\mcA_0}$ which is the strict module map sending $x \in \mcA_+ \left( \Lambda_k, \Lambda_n \right)$ to 
	\[h(x) = s \pi \left( x \right) \in \mcA_0 \left( \Lambda_k, \Lambda_n \right) \left[ 1 \right] \subset \pi^* \mcM_{\mcA_0} \left( \Lambda_k \right) \]
	($s : \mcA_0 \left( \Lambda_k, \Lambda_n \right) \to \mcA_0 \left( \Lambda_k, \Lambda_n \right) \left[ 1 \right]$ is the usual degree $(-1)$ map).
	According to Proposition \ref{prop morphism induced by homotopy}, this induces a closed $\mcA_+$-module map $t_0 : \mcM_{\mcA_+} \to \pi^* \mcM_{\mcA_0}$. Moreover, the following diagram of $\mcA_+$-modules is commutative
	\[\begin{tikzcd}
	\mcA_+ \left( - , \Lambda \right) \ar[d, "t_{\mcA_+}"] \ar[r, "t_{\pi}"] & \pi^* \mcA_0 \left( - , \Lambda  \right) \ar[d, "\pi^* t_{\mcA_0}"] \\
	\mcM_{\mcA_+} \ar[r, "t_0"] & \pi^* \mcM_{\mcA_0} .
	\end{tikzcd} \] 
	
	Now according to Proposition \ref{prop quasi-isomorphism between localizations}, there is a chain map $u : \, _{W_+^{-1}} \mcM_{\mcA_+} \left( \Lambda \right) \to \, _{W_0^{-1}} \mcM_{\mcA_0} \left( \Lambda \right)$ such that the following diagram of chain complexes commutes
	\[\begin{tikzcd}
	\mcA_+ \left[ W_+^{-1} \right] \left( \Lambda , \Lambda \right) \ar[d, "_{W_+^{-1}} t_{\mcA_+}"] \ar[r, "\widetilde{\pi}"] & \mcA_0 \left[ W_0^{-1} \right] \left( \Lambda , \Lambda \right) \ar[d, "_{W_0^{-1}} t_{\mcA_0}"] \\
	_{W_+^{-1}} \mcM_{\mcA_+} \left( \Lambda \right) \ar[r, "u"] & _{W_0^{-1}} \mcM_{\mcA_0} \left( \Lambda \right) \\
	\mcM_{\mcA_+} \left( \Lambda \right) \ar[u, hook] \ar[r, "t_0"] & \mcM_{\mcA_0} \left( \Lambda \right) \ar[u, hook]
	\end{tikzcd} \]
	(the two vertical maps on the bottom are the inclusions). 
	Moreover, the inclusions 
	\[\overline{LA^*} \left( \Lambda \right) \hookrightarrow LA_+^* \left( \Lambda \right), \, \overline{LA^*} \left( \Lambda \right) \hookrightarrow \, _{W_+^{-1}} \mcM_{\mcA_+} \left( \Lambda \right), \, \overline{LA^*} \left( \Lambda \right) \hookrightarrow \mcM_{\mcA_+} \left( \Lambda \right) \]
	make the following diagram commutes 
	\[\begin{tikzcd}
	\overline{LA^*} \left( \Lambda \right) \ar[r, hook] \ar[d, equal] & LA_+^* \left( \Lambda \right) \ar[d, "_{W_+^{-1}} t_{\mcA_+}"] \ar[r, "\widetilde{\pi}"] & LA_0^* \left( \Lambda \right) \ar[d, "_{W_0^{-1}} t_{\mcA_0}"] \\
	\overline{LA^*} \left( \Lambda \right) \ar[r, hook] \ar[d, equal] & _{W_+^{-1}} \mcM_{\mcA_+} \left( \Lambda \right) \ar[r, "u"] & _{W_0^{-1}} \mcM_{\mcA_0} \left( \Lambda \right) \\
	\overline{LA^*} \left( \Lambda \right) \ar[r, hook] & \mcM_{\mcA_+} \left( \Lambda \right) \ar[u, hook] \ar[r, "t_0"] & \mcM_{\mcA_0} \left( \Lambda \right) \ar[u, hook] .
	\end{tikzcd} \]
	According to Lemma \ref{lemma multiplication by the minimum in the different versions}, $\mcA_+$ and $\mcA_0$ satisfy the hypotheses of Lemma \ref{lemma second result for specific module}. Thus, using Lemma \ref{lemma second result for specific module} and Proposition \ref{prop quasi-iso between a module and its localization}, we know that the vertical maps are quasi-isomorphisms. Therefore, we get the following commutative diagram of chain complexes
	\[\begin{tikzcd}
	\overline{LA^*} \left( \Lambda \right) \ar[r, "\phi"] \ar[d, equal] & \mathrm{Cone} \left( LA_+^* \left( \Lambda \right) \xrightarrow{\widetilde{\pi}} LA_0^* \left( \Lambda \right) \right) \ar[d, "\sim"] \\
	\overline{LA^*} \left( \Lambda \right) \ar[r] \ar[d, equal] & \mathrm{Cone} \left( _{W_+^{-1}} \mcM_{\mcA_+} \left( \Lambda \right) \xrightarrow{u} \, _{W_0^{-1}} \mcM_{\mcA_0} \left( \Lambda \right) \right) \\
	\overline{LA^*} \left( \Lambda \right) \ar[r, "\psi"] & \mathrm{Cone} \left( \mcM_{\mcA_+} \left( \Lambda \right) \xrightarrow{t_0} \mcM_{\mcA_0} \left( \Lambda \right) \right) \ar[u, "\sim" right] .
	\end{tikzcd} \]
	Therefore, in order to show that 
	\[\phi : \overline{LA^*} \left( \Lambda \right) \to \mathrm{Cone} \left( LA_+^* \left( \Lambda \right) \xrightarrow{\widetilde{\pi}} LA_0^* \left( \Lambda \right) \right) \]
	is a quasi-isomorphism, it suffices to show that 
	\[\psi : \overline{LA^*} \left( \Lambda \right) \to \mathrm{Cone} \left( \mcM_{\mcA_+} \left( \Lambda \right) \xrightarrow{t_0} \mcM_{\mcA_0} \left( \Lambda \right) \right) \]
	is a quasi-isomorphism. Observe that the inclusion $\ker \left( t_0 \right) \hookrightarrow \mathrm{Cone} (t_0)$ is a quasi-isomorphism because $t_0$ is surjective. Thus it suffices to show that the inclusion $\overline{LA^*} \left( \Lambda \right) \hookrightarrow \ker \left( t_0 \right)$ is a quasi-isomorphism.
	Recall that we denote by $\mcA_{long} \left( \Lambda_m, \Lambda_n \right)$ the subcomplex of $\mcA_+ \left( \Lambda_m, \Lambda_n \right)$ generated by $\mcR_{long} \left( \Lambda_m, \Lambda_n \right)$. Then observe that $\overline{LA^*} \left( \Lambda \right) = \mcA_{long} \left( \Lambda, \Lambda \right)$ and 
	\[\ker \left( t_0 \right) = \left[
	\begin{tikzcd}
	\mcA_{long} \left( \Lambda , \Lambda_0 \right) \ar[d, "\mathrm{id}"] \ar[rd, "t_{c_0}"] & \mcA_{long} \left( \Lambda , \Lambda_1 \right) \ar[d, "\mathrm{id}"] \ar[rd, "t_{c_1}"] & \dots \\
	\mcA_{long} \left( \Lambda , \Lambda_0 \right) & \mcA_{long} \left( \Lambda , \Lambda_1 \right) & \dots
	\end{tikzcd} 
	\right] . \]
	Thus the result follows from Lemmas \ref{lemma multiplication by the minimum in the different versions} and \ref{lemma first result for specific module}. 
	

\end{proof}

==> Makefile <==
.PHONY: all viewpdf pdf clean

TARGET       = main
SOURCE_FILES = $(TARGET).tex $(wildcard */*.tex)
BIB_FILES    = $(wildcard biblio/*.bib)
FIGURES      = $(wildcard */figures/*)

# Set the pdf reader according to the operating system
OS = $(shell uname)
ifeq ($(OS), Darwin)
	PDF_READER = open
endif
ifeq ($(OS), Linux)
	PDF_READER = evince
endif

all: pdf

viewpdf: pdf
	$(PDF_READER) $(TARGET).pdf &

pdf: $(TARGET).pdf

$(TARGET).pdf: $(SOURCE_FILES) $(BIB_FILES) $(FIGURES) these-dbl.cls
	pdflatex -interaction=nonstopmode -jobname=$(TARGET) $(SOURCE_FILES)
	biber $(TARGET)
	pdflatex -interaction=nonstopmode -jobname=$(TARGET) $(SOURCE_FILES) # For biber

clean:
	rm -f $(TARGET).{ps,pdf,bcf,run.xml}
	for suffix in dvi aux bbl blg toc ind out brf ilg idx synctex.gz log; do \
		find . -type d -name ".git" -prune -o -type f -name "*.$${suffix}" -print -exec rm {} \;  ; \
	done

